Residual Degradation Learning Unfolding Framework with Mixing Priors across Spectral and Spatial for Compressive Spectral Imaging

To acquire a snapshot spectral image, coded aperture snapshot spectral imaging (CASSI) is proposed. A core problem of the CASSI system is to recover the reliable and fine underlying 3D spectral cube from the 2D measurement. By alternately solving a data subproblem and a prior subproblem, deep unfolding methods achieve good performance. However, in the data subproblem, the used sensing matrix is ill-suited for the real degradation process due to the device errors caused by phase aberration, distortion; in the prior subproblem, it is important to design a suitable model to jointly exploit both spatial and spectral priors. In this paper, we propose a Residual Degradation Learning Unfolding Framework (RDLUF), which bridges the gap between the sensing matrix and the degradation process. Moreover, a Mix$S^2$ Transformer is designed via mixing priors across spectral and spatial to strengthen the spectral-spatial representation capability. Finally, plugging the Mix$S^2$ Transformer into the RDLUF leads to an end-to-end trainable neural network RDLUF-Mix$S^2$. Experimental results establish the superior performance of the proposed method over existing ones.

==> tables/table2.tex <==
\begin{table}[!htbp]
    \centering
    \scalebox{0.60}{
        \begin{tabular}{c c c  c c c c}
        		%\small
        		\toprule
        		Spectral Branch & Spatial Branch & Spectral Interaction  & Spatial Interaction & PSNR & SSIM \\
        		\midrule
        		\checkmark & & & &37.17 &0.961 \\
        		\checkmark  & \checkmark & & &37.41 &0.962 \\
        		\checkmark & \checkmark &\checkmark & & 37.48 &0.962 \\
        		\checkmark & \checkmark &  & \checkmark & 37.49 & 0.962 \\
        		\checkmark & \checkmark & \checkmark & \checkmark &\bf 37.56 & \bf0.963 \\
        		\bottomrule
        \end{tabular}
    }
    \vspace{-3.0mm}
    \caption{\small Break-down ablation studies for Mix$S^2$ structure.}
% 	\caption{\small Break-down ablation studies for Mix$S^2$ structure. Every component boosts to higher performance.}
    \label{tab:table2}
    \vspace{-3.0mm}
\end{table}

==> tables/table3.tex <==
\begin{table}[!htbp]
    \centering
    \scalebox{0.6}{
        \begin{tabular}{c c c  c c c c}
        		%\small
        		\toprule
        		Residual Degradation Learning  & PSNR & SSIM\\
        		\midrule
        		w/o  & 36.87 & 0.958 \\
        		w &\bf 37.56 &\bf 0.963 \\
        		\bottomrule
        \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{\small Ablation of RDLGD module.}
    \label{tab:table3}
    \vspace{-0.3cm}
\end{table}

==> tables/table4.tex <==
\begin{table}[!htbp]
    \centering
    \scalebox{0.6}{
        \begin{tabular}{c c c  c c c c}
        		%\small
        		\toprule
        		Stage Interaction & Block Interaction  & PSNR & SSIM \\
        		\midrule
        		& & 37.41 & 0.957 \\
        		\checkmark & & 37.49 & 0.960 \\
        		& \checkmark & 37.50 & 0.961 \\
        		\checkmark & \checkmark & \textbf{37.56} & \textbf{0.963} \\
        		\bottomrule
        \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{\small Ablation to study the effect of Stage Interaction and Block Interaction.}
    \label{tab:table4}
    \vspace{-0.3cm}
\end{table}

==> tables/table_poster.tex <==
\begin{table*}[t]
    \renewcommand{\arraystretch}{2} 
    \resizebox{0.99\textwidth}{!}
    {
        \begin{tabular}{c|c c c c c c c c c}
            \toprule
            \hline
            Metric & DGSMP [1] & HDNet [2] & MST-L [3] & CST-L* [4] & DAUHST-9stg [5] & Ours 3stg & Ours 5stg & Ours 7stg & Ours 9stg \\
            \hline
            PSNR & 32.63 & 34.97 & 35.18 & 36.12 & 38.36 & 37.56 & 38.59 & 39.35 & \textbf{39.57} \\
            \hline
            SSIM & 0.917 & 0.943 & 0.948 & 0.957 & 0.967 & 0.963 & 0.969 & 0.973 & \textbf{0.974} \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:poster}
\end{table*}

==> tables/table_test.tex <==
\begin{table}[!htbp]
    \centering
    \scalebox{0.8}{
        \begin{tabular}{c c c  c c c c}
        		%\small
        		\toprule
        		Mask Type  & PSNR & SSIM\\
        		\midrule
        		Uniform mask  & 37.10 & 0.956 \\
        		Gaussian mask & 37.30 & 0.959 \\
        		Real mask & 37.56 & 0.963 \\
        		Optimized binary mask &\bf 37.78 &\bf 0.965\\
        		\bottomrule
        \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{\small Ablation of number of stages. * notes all parameters is independent.}
    \label{tab:test}
    \vspace{-0.3cm}
\end{table}
